New structurally unstable families of planar vector fields

We study global bifurcations in generic 3-parameter families of vector fields on $S^2$. In the recent article [arXiv:1506.06797], Ilyashenko, Kudryashov, and Schurov show that 3-parameter unfoldings of vector fields with the polycycle "tears of the heart" are structurally unstable. We consider 3-parameter unfoldings of vector fields with separatrix graphs "ears" and "glasses", and prove that these families are structurally unstable as well. We also study in more details the classical bifurcation of a saddle loop, and use it as a building block in our main example.

==> asy/ears-glasses-nolua-1.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-136.391467,73.491748)(-0.292893,-1.000000){ }%


==> asy/ears-glasses-nolua-2.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-2_0.pdf}%
}%


==> asy/ears-glasses-nolua-3.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-3_0.pdf}%
}%


==> asy/ears-glasses-nolua-4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-4_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-3.887403,5.610415)(-0.500000,-1.000000){\(\varepsilon\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-241.034018,85.972422)(-1.000000,0.000000){\(O\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-267.357499,80.831897)(-0.500000,-1.000000){\(\Gamma\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-125.093719,80.831897)(-0.500000,-1.000000){\(\Gamma\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-106.088783,81.713871)(-1.000000,-1.000000){\(S\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-83.551988,81.713871)(0.000000,-1.000000){\(U\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-94.820386,86.854397)(-0.500000,0.000000){\(\varepsilon\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-199.420229,17.574404)(-0.500000,0.000000){\(\varepsilon=0\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-57.156449,17.574404)(-0.500000,0.188809){\(\varepsilon=\varepsilon_n>0\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-341.684008,17.574404)(-0.500000,0.057199){\(\varepsilon<0\)}%


==> asy/ears-glasses-nolua-5.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-5_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-95.658035,51.318039)(-1.000000,0.000000){\(L\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-48.720350,51.318039)(0.000000,0.000000){\(R\)}%


==> asy/ears-glasses-nolua-6.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-6_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-95.815366,51.318039)(-1.000000,0.000000){\(L\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-48.877682,47.059489)(0.000000,-1.000000){\(R\)}%


==> asy/ears-glasses-nolua-7.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-7_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-257.838743,7.749315)(-1.000000,-1.000000){\(0\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-157.547460,6.867340)(-0.500000,-1.000000){\(\varepsilon\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-258.720718,137.915992)(-1.000000,-0.500000){\(\delta\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-364.536578,76.026566)(-1.000000,0.000000){\(L\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-317.598894,76.026566)(0.000000,0.000000){\(R\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-405.599761,65.907072)(-1.000000,0.000000){\(\varepsilon\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-276.535711,65.907072)(0.000000,0.000000){\(\delta\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-341.067736,76.908541)(-0.500000,0.000000){\(\sigma\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-341.067736,28.206907)(-0.500000,-1.000000){\(\varepsilon=\delta=0\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-249.302917,204.063968)(-1.000000,0.000000){\(L\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-202.365232,204.063968)(0.000000,0.000000){\(R\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-225.834074,159.255559)(-0.500000,-0.241629){\(\varepsilon=\varepsilon_n\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-95.658035,97.366133)(-1.000000,0.000000){\(L\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-48.720350,97.366133)(0.000000,0.000000){\(R\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-72.189192,49.546474)(-0.500000,-0.822370){\(\delta=\delta_m\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-95.658035,204.063968)(-1.000000,0.000000){\(L\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-48.720350,204.063968)(0.000000,0.000000){\(R\)}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{10.037500}{12.045000}\selectfont
\ASYalign(-72.189192,156.244309)(-0.500000,-0.945880){\(\alpha\in\mathcal E\)}%

